A Tutorial on Beam Management for 3GPP NR at mmWave Frequencies

The millimeter wave (mmWave) frequencies offer the availability of huge bandwidths to provide unprecedented data rates to next-generation cellular mobile terminals. However, mmWave links are highly susceptible to rapid channel variations and suffer from severe free-space pathloss and atmospheric absorption. To address these challenges, the base stations and the mobile terminals will use highly directional antennas to achieve sufficient link budget in wide area networks. The consequence is the need for precise alignment of the transmitter and the receiver beams, an operation which may increase the latency of establishing a link, and has important implications for control layer procedures, such as initial access, handover and beam tracking. This tutorial provides an overview of recently proposed measurement techniques for beam and mobility management in mmWave cellular networks, and gives insights into the design of accurate, reactive and robust control schemes suitable for a 3GPP NR cellular network. We will illustrate that the best strategy depends on the specific environment in which the nodes are deployed, and give guidelines to inform the optimal choice as a function of the system parameters.

==> figures/single_burst.tex <==
\begin{table}[t]
\small
  \centering
  %\setlength\belowcaptionskip{-0.4cm}
    \renewcommand{\arraystretch}{1}% Tighter
  \begin{tabular}{@{}c|cccccc|c@{}}
  \toprule
  	& \multicolumn{6}{c|}{$M_{\gls{gnb}} \times M_{\gls{ue}}$} & \\
	$N_{\rm SS}$ & $4\times4$ & $16\times4$ & $64\times4$ & $16\times16$ & $64\times16$ & $64\times1$ & Beamforming options \\
	\midrule
	\multirow{4}{*}{$8$}		& 0 &	0 &	0 &	0 &	0 &	0 &  Both analog \\
			& 1 &	0 &	0 &	0 &	0 &	0 & \gls{gnb} analog, \gls{ue} hybrid\\
			& 1	&   0 &	0 &	0 &	0 &	0 & \gls{gnb} analog, \gls{ue} digital\\
			& 1 &	1 &	1 &	0 &	0 &	1 & \gls{gnb} digital, \gls{ue} analog\\
			\midrule
	\multirow{4}{*}{$16$}		& 1 &	0 &	0 &	0 &	0 &	0 & Both analog \\
			& 1 &	0 &	0 &	0 &	0 &	0 & \gls{gnb} analog, \gls{ue} hybrid\\
			& 1	&   0 &	0 &	0 &	0 &	0 & \gls{gnb} analog, \gls{ue} digital\\
			& 1 &	1 &	1 &	0 &	0 &	1 & \gls{gnb} digital, \gls{ue} analog\\
			\midrule
	\multirow{4}{*}{$32$}		& 1 &	0 &	0 &	0 &	0 &	0 & Both analog \\
			& 1 &	0 &	0 &	0 &	0 &	0 & \gls{gnb} analog, \gls{ue} hybrid\\
			& 1	&   1 &	0 &	0 &	0 &	0 & \gls{gnb} analog, \gls{ue} digital\\
			& 1 &	1 &	1 &	0 &	0 &	1 & \gls{gnb} digital, \gls{ue} analog\\
			\midrule
	\multirow{4}{*}{$64$}		& 1 &	0 &	0 &	0 &	0 &	1 & Both analog \\
			& 1 &	1 &	0 &	0 &	0 &	1 & \gls{gnb} analog, \gls{ue} hybrid\\
			& 1 &	1 &	0 &	1 &	0 &	1 & \gls{gnb} analog, \gls{ue} digital\\
			& 1 &	1 &	1 &	1 &	1 &	1 & \gls{gnb} digital, \gls{ue} analog\\
	\bottomrule
	\end{tabular}
	\caption{Configurations of beamforming solutions, antenna arrays size $M_{\gls{gnb}} \times M_{\gls{ue}}$, and \gls{ss} blocks per burst $N_{\rm SS}$ that makes it possible to sweep all the directions in an \gls{ss} burst. A $1$ indicates that a single burst is enough, a $0$ otherwise.}
	\label{table:ia_config}
\end{table}

